BDIViz: An Interactive Visualization System for Biomedical Schema Matching with LLM-Powered Validation

Biomedical data harmonization is essential for enabling exploratory analyses and meta-studies, but the process of schema matching - identifying semantic correspondences between elements of disparate datasets (schemas) - remains a labor-intensive and error-prone task. Even state-of-the-art automated methods often yield low accuracy when applied to biomedical schemas due to the large number of attributes and nuanced semantic differences between them. We present BDIViz, a novel visual analytics system designed to streamline the schema matching process for biomedical data. Through formative studies with domain experts, we identified key requirements for an effective solution and developed interactive visualization techniques that address both scalability challenges and semantic ambiguity. BDIViz employs an ensemble approach that combines multiple matching methods with LLM-based validation, summarizes matches through interactive heatmaps, and provides coordinated views that enable users to quickly compare attributes and their values. Our method-agnostic design allows the system to integrate various schema matching algorithms and adapt to application-specific needs. Through two biomedical case studies and a within-subject user study with domain experts, we demonstrate that BDIViz significantly improves matching accuracy while reducing cognitive load and curation time compared to baseline approaches.

==> comments/clean.tex <==
\newcommand{\eden}[1]{\textcolor{cyan}{}}
\newcommand{\hide}[1]{}
\newcommand{\dt}[1]{\textcolor{magenta}{}}
\newcommand{\jf}[1]{{\color{green}{}}}

\newcommand{\claudio}[1]{{\color{blue} }}
\newcommand{\guande}[1]{\textcolor[HTML]{FFC0CB}{}} % John's color


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tables/desiderata.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{|c|p{6.5cm}|c|}
\hline
\textbf{No.} & \textbf{Desiderata Description} & \textbf{Imp.} \\
\hline
R1 & \textbf{Efficient match discovery:} All experts highlighted the challenge of manually comparing large schemas and preferred a system that automatically surfaces potential matches, reducing the need for tedious one-by-one inspection. & \criticalicon \\
\hline
R2 & \textbf{Accepting/Rejecting matches:} Experts need the ability to manually accept or reject matches. E1, E2, and E3, said they wanted the capability to exclude attributes that do not have any valid matches from the task entirely. & \criticalicon \\
\hline
R3 & \textbf{Value comparisons:} All experts emphasized that comparing unique values within each categorical attribute is crucial for determining correct matches. & \criticalicon \\
\hline
R4 & \textbf{Value distribution insights:} E2 and E3 emphasized the need for understanding value distributions in both source and target datasets, particularly for categorical and numerical attributes, to aid accurate schema matching. & \importanticon \\
\hline
R5 & \textbf{Filtering capabilities:} E2 and E4 highlighted the need for a filtering option to exclude matching candidates based on datatype or similarity score generated by the recommendation model. & \importanticon  \\
\hline
R6 & \textbf{History of actions:} E1 emphasized the need maintaining a record of their selections and actions, undo/redo capabilities to track actions, correct errors, and support iterative exploration and refinement, as users get more familiar with the data. & \importanticon  \\
% Expert E1 emphasized the importance of maintaining a record of their selections and actions, with the ability to undo mistakes and redo actions as needed. These functionalities are crucial for any exploratory task, as errors are easy to make, and refinements often become necessary as users grow more familiar with the data. Incorporating undo/redo capabilities not only supports error correction but also encourages iterative exploration and refinement, as seen in tools like Vizier and VisTrails [\dt{REF}]. & \importanticon  \\
\hline
R7 & \textbf{Multi-Source Comparison:} E1 emphasized the need to compare multiple source datasets simultaneously, particularly for mapping similar columns across datasets like CPTAC. & \optionalicon  \\
\hline
\end{tabular}
\vspace{- 7 pt}
\caption{Schema Matching Requirements and their Importance. represents the critical desiderata.}
\label{tab:desiderata}
\end{table}

% Add these to the preamble of your document:
% \usepackage{graphicx}
% \usepackage{xcolor}
% \usepackage{array}

==> tables/designconsiderations.tex <==
\begin{table}[h!] 
\centering
\small
\begin{tabular}{|c|p{6.5cm}|}
\hline
\textbf{No.} & \textbf{Final Design Considerations} \\
\hline
DC1 \label{dr:desiderata} & \textbf{Enabling efficient schema matching by implementing all the desiderata in Table~\ref{tab:desiderata}:} Our system should support key requirements from formative studies, including automated matching, interactive refinement, and transparent reasoning to aid complex database integration tasks.\\
\hline
DC2 \label{dr:agent} & \textbf{Enabling the LLM agent to learn from human feedback for efficient and effective matching correction:} The system should have a learning mechanism that adapts based on user feedback, improving matching accuracy and efficiency over time. \\
\hline
DC3\label{dr:intuitive} & \textbf{Enabling intuitive representation of schema ontology and relationships for user comprehension:} The visualization should communicate hierarchical relationships between database columns, aiding users in identifying patterns and understanding the structural context of matches. \\
\hline
DC4 \label{dr:additional} & \textbf{Providing additional information including value matching and knowledge base to support decision-making:} Beyond similarity scores, the system should present value matching and domain-specific knowledge to help users make informed decisions, especially when column names or metadata are insufficient. \\
\hline

\end{tabular}

\vspace{- 7 pt}
\caption{\dt{to update - guande} Final design considerations}
\label{tab:designconsiderations}
\end{table}



==> tables/experts.tex <==
\begin{table}[h!]
\centering
\small % Reduces the font size for the entire table

\begin{tabular}{|p{0.1cm}|p{2.4cm}|p{5.1cm}|}
\hline
\textbf{} & \textbf{Title} & \textbf{Background} \\
\hline
E1 & Staff Researcher \& Scientific Programmer at Biomedical Data Lab, Medical Institute & E1 collaborates with scientists on projects, including computer vision \& image analysis, statistical modeling, biological systems simulations, data repositories creation, \& clinical data informatics. \\
\hline
E2 & Staff Research Scientist, at Biomedical Data Lab, Medical Institute & E2 conducts computational experiments on high-throughput cancer genomics data \& develops statistical \& data-mining methods for exploratory analysis. \\
\hline
E3 & PhD Cand. Data Scientist, at Biomedical Data Lab, Medical Institute & E3 develops deep learning-based computational tools for spatial multi-omics, focusing on data simulation, context reconstruction, \& integration. \\
\hline
E4 & Principal Data Scientist, at a Major Research Organization & E4 has 15+ years of experience of leading various biomedical data integration and harmonization initiatives. \\
\hline
E5 & Data Librarian, Head of Data Sharing \& Metadata Management, at Medical Library of a Medical Institution & E5 ensures seamless dataset integration across biomedical systems by mapping metadata schemas for interoperability. E5 collaborates across institutions \& conducts interviews to align metadata standards. \\
\hline
\end{tabular}
\vspace{- 7 pt}
\caption{Experts in biomedical data research who participated in the formative study, their titles, and backgrounds}
\label{tab:experts}
\vspace{-.3cm}
\end{table}

==> tables/sus.tex <==
% \begin{table*}[t]
% \caption{System Usability Scale (SUS) Results Comparison between BDIViz and Baseline}
% % \label{tab:sus-results}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccp{0.12\textwidth}}
% \toprule
% \textbf{Statement} & \multicolumn{2}{c}{\textbf{BDIViz}} & \multicolumn{2}{c}{\textbf{Baseline}} & \textbf{U} & \textbf{p-value} & \textbf{Effect size (r)} & \textbf{\% Change} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & \textbf{Mean} & \textbf{Median} & \textbf{Mean} & \textbf{Median} & & & & \\
% \midrule
% I think I would like to use this system frequently & 5.25 & 5.00 & 2.83 & 2.00 & 117.0 & 0.0092** & 0.5303 & +85.29\% \\
% I found the system unnecessarily complex & 2.33 & 2.00 & 5.17 & 5.50 & 10.0 & 0.0003*** & 0.7307 & -54.84\% \\
% I thought the system was easy to use & 5.50 & 6.00 & 3.50 & 3.00 & 112.0 & 0.0195** & 0.4714 & +57.14\% \\
% I found the various functions in this system well integrated & 5.92 & 6.00 & 2.75 & 2.50 & 133.5 & 0.0004*** & 0.7248 & +115.15\% \\
% I thought there was too much inconsistency in this system & 2.33 & 2.50 & 5.08 & 5.50 & 21.5 & 0.0034** & 0.5951 & -54.10\% \\
% I found the system very cumbersome to use & 2.83 & 3.00 & 4.75 & 5.00 & 34.5 & 0.0297* & 0.4419 & -40.35\% \\
% \midrule
% \multicolumn{9}{l}{\textbf{Additional Usability Metrics}} \\
% \midrule
% I think I can integrate the system in my current workflow & 5.50 & 6.00 & 3.67 & 3.50 & 107.0 & 0.0432* & 0.4125 & +50.00\% \\
% I think I was engaged in using the system & 5.83 & 6.00 & 4.00 & 4.50 & 111.0 & 0.0234* & 0.4596 & +45.83\% \\
% % I think the initially-generated matching result is clear and accurate & 4.75 & 5.00 & 3.17 & 3.00 & 121.5 & 0.0037** & 0.5834 & +50.00\% \\
% % I think the presented visualizations help me understand the database & 5.58 & 5.50 & 3.75 & 4.00 & 116.0 & 0.0098** & 0.5185 & +48.89\% \\
% % I believe the explanation-based interaction is helpful for schema matching & 6.00 & 6.00 & 3.67 & 4.00 & 124.5 & 0.0018** & 0.6187 & +63.64\% \\
% I think after the interaction, I achieve better matching results & 5.83 & 6.00 & 4.08 & 4.00 & 112.0 & 0.0197* & 0.4714 & +42.86\% \\
% I think the overall workflow can make my workflow more efficient & 5.75 & 6.00 & 3.42 & 3.00 & 122.5 & 0.0034** & 0.5951 & +68.29\% \\
% \bottomrule
% \multicolumn{9}{l}{\footnotesize \textit{Note:} All metrics measured on a 7-point Likert scale (1=strongly disagree, 7=strongly agree). N=12 for all conditions.} \\
% \multicolumn{9}{l}{\footnotesize Significance levels: * p < 0.05,  **p < 0.01, ***p < 0.001} \\
% \end{tabular}}
% \vspace{ -15 pt}
% \label{tab:sus}
% \end{table*}

\begin{table}[h!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Statement} & \multicolumn{2}{c}{\textbf{Mean}} & \multirow{2}{*}{\textbf{U}} & \multirow{2}{*}{\textbf{p-value}} & \multirow{2}{*}{\textbf{r}} \\
\cmidrule(lr){2-3}
& \textbf{BDIViz} & \textbf{Baseline} & & & \\
\midrule
Would use frequently & 5.25 & 2.83 & 117.0 & 0.009** & 0.53 \\
Not unnecessarily complex & 5.67 & 2.83 & 10.0 & <0.001*** & 0.73 \\
Easy to use & 5.50 & 3.50 & 112.0 & 0.020* & 0.47 \\
Well integrated functions & 5.92 & 2.75 & 133.5 & <0.001*** & 0.72 \\
Consistent system & 5.67 & 2.92 & 21.5 & 0.003** & 0.60 \\
Not cumbersome to use & 5.17 & 3.25 & 34.5 & 0.030* & 0.44 \\
\midrule
\multicolumn{6}{l}{\textbf{Additional Usability Metrics}} \\
\midrule
Integrates with workflow & 5.50 & 3.67 & 107.0 & 0.043* & 0.41 \\
Engaging to use & 5.83 & 4.00 & 111.0 & 0.023* & 0.46 \\
Achieved better results & 5.83 & 4.08 & 112.0 & 0.020* & 0.47 \\
More efficient workflow & 5.75 & 3.42 & 122.5 & 0.003** & 0.60 \\
\bottomrule
\multicolumn{6}{p{0.95\columnwidth}}{\footnotesize \textit{Note:} All metrics on 7-point Likert scale (1=strongly disagree, 7=strongly agree). N=12 for all conditions. Negative statements were inverted for consistency. Significance: * p < 0.05, **p < 0.01, ***p < 0.001}
\end{tabular}}
\vspace{-.3cm}
\caption{System Usability Scale (SUS) Results: BDIViz vs. Baseline}
\label{tab:sus}
\vspace{-.1cm}
\end{table}
